The Fine Structure of the Singular Set of Area-Minimizing Integral Currents III: Frequency 1 Flat Singular Points and $\mathcal{H}^{m-2}$-a.e. Uniqueness of Tangent Cones

We consider an area-minimizing integral current $T$ of codimension higher than 1 ins a smooth Riemannian manifold $\Sigma$. We prove that $T$ has a unique tangent cone, which is a superposition of planes, at $\mathcal{H}^{m-2}$-a.e. point in its support. In combination with works of the first and third authors, we conclude that the singular set of $T$ is countably $(m-2)$-rectifiable.

==> bibliography.tex <==
\begin{bibdiv}
    \begin{biblist}
        
                \bib{DL-All}{incollection}{
    AUTHOR = {De Lellis, Camillo},
     TITLE = {Allard's interior regularity theorem: an invitation to
              stationary varifolds},
 BOOKTITLE = {Nonlinear analysis in geometry and applied mathematics. {P}art
              2},
    SERIES = {Harv. Univ. Cent. Math. Sci. Appl. Ser. Math.},
    VOLUME = {2},
     PAGES = {23--49},
 PUBLISHER = {Int. Press, Somerville, MA},
      YEAR = {2018},
   %MRCLASS = {49Q15 (35B65)},
  %MRNUMBER = {3823880},
%MRREVIEWER = {Andreas Gastel},
}

       \bib{Spolaor_15}{article}{
             AUTHOR = {Spolaor, Luca},
             TITLE = {Almgren's type regularity for semicalibrated currents},
             JOURNAL = {Adv. Math.},
             %FJOURNAL = {Advances in Mathematics},
             VOLUME = {350},
             YEAR = {2019},
             PAGES = {747--815},
             ISSN = {0001-8708},
             %MRCLASS = {49Q15 (49N60)},
             %MRNUMBER = {3948685},
             %MRREVIEWER = {Alp\'{a}r R. M\'{e}sz\'{a}ros},
             DOI = {10.1016/j.aim.2019.04.057},
             URL = {https://doi.org/10.1016/j.aim.2019.04.057},
         }

        \bib{Allard_72}{article}{
            AUTHOR = {Allard, William K.},
            TITLE = {On the first variation of a varifold},
            JOURNAL = {Ann. of Math. (2)},
            %FJOURNAL = {Annals of Mathematics. Second Series},
            VOLUME = {95},
            YEAR = {1972},
            PAGES = {417--491},
            ISSN = {0003-486X},
            %MRCLASS = {49F20},
            %MRNUMBER = {307015},
            %MRREVIEWER = {M. Klingmann},
            DOI = {10.2307/1970868},
            URL = {https://doi.org/10.2307/1970868},
        }
        
        \bib{Almgren_regularity}{book}{
            AUTHOR = {Almgren Jr., Frederick J.},
            TITLE = {Almgren's big regularity paper},
            SERIES = {World Scientific Monograph Series in Mathematics},
            VOLUME = {1},
            NOTE = {$Q$-valued functions minimizing Dirichlet's integral and the
                regularity of area-minimizing rectifiable currents up to
                codimension 2,
                With a preface by Jean E. Taylor and Vladimir Scheffer},
            PUBLISHER = {World Scientific Publishing Co., Inc., River Edge, NJ},
            YEAR = {2000},
            PAGES = {xvi+955},
            ISBN = {981-02-4108-9},
            %MRCLASS = {49-02 (35J20 49N60 49Q20 58E12)},
            %MRNUMBER = {1777737},
            %MRREVIEWER = {Brian Cabell White},
        }
        
%         \bib{AT15}{article}{
%             AUTHOR = {Azzam, Jonas},
%             author = {Tolsa, Xavier},
%             TITLE = {Characterization of {$n$}-rectifiability in terms of {J}ones'
%               square function: {P}art {II}},
%             JOURNAL = {Geom. Funct. Anal.},
%             VOLUME = {25},
%             YEAR = {2015},
%             NUMBER = {5},
%             PAGES = {1371--1412},
%             ISSN = {1016-443X},
%             DOI = {10.1007/s00039-015-0334-7},
%             URL = {https://doi.org/10.1007/s00039-015-0334-7},
%         }
        
         \bib{SXChang}{article}{
             AUTHOR = {Chang, Sheldon Xu-Dong},
             TITLE = {Two-dimensional area minimizing integral currents are
                 classical minimal surfaces},
             JOURNAL = {J. Amer. Math. Soc.},
             %FJOURNAL = {Journal of the American Mathematical Society},
             VOLUME = {1},
             YEAR = {1988},
             NUMBER = {4},
             PAGES = {699--778},
             ISSN = {0894-0347},
             %MRCLASS = {49F20 (49F10 49F22 58E12 58E15)},
             %MRNUMBER = {946554},
             %MRREVIEWER = {Harold Parks},
             DOI = {10.2307/1990991},
             URL = {https://doi.org/10.2307/1990991},
         }
        
%     \bib{DL_JDG}{article}{
%         title={The size of the singular set of area-minimizing currents},
%         author={De Lellis, Camillo},
%         journal={arXiv preprint arXiv:1506.08118},
%         year={2015}
%         }
        
%     \bib{DLDPHM}{article}{
% 		AUTHOR = {De Lellis, Camillo},
% 		author={De Philippis, Guido},
% 		author={Hirsch, Jonas},
% 		author={Massaccesi, Annalisa},
% 		TITLE = {Boundary regularity of mass-minimizing integral currents and a question of {A}lmgren},
% 		BOOKTITLE = {2017 {MATRIX} annals},
% 		SERIES = {MATRIX Book Ser.},
% 		VOLUME = {2},
% 		PAGES = {193--205},
% 		PUBLISHER = {Springer, Cham},
% 		YEAR = {2019},
% 		%MRCLASS = {53C42 (35B65 35R01 49Q15 58A25)},
% 		%MRNUMBER = {3931066},
% 		%MRREVIEWER = {Fei-Tsen Liang},
% 	}


\bib{DLHMS}{article}{
	author={De Lellis, Camillo},
	author={Hirsch, Jonas},
	author={Marchese, Andrea},
	author={Stuvard, Salvatore},
	title={Regularity of area minimizing currents mod p},
	journal={Geometric and Functional Analysis},
	year={2020}
}

	\bib{DLHMSS}{article}{
		author = {De Lellis, Camillo},
		author={Hirsch, Jonas},
		author={Marchese, Andrea},
		author={Spolaor, Luca},
		author={Stuvard, Salvatore},
		title = {Area minimizing hypersurfaces modulo $p$: a geometric free-boundary problem},
		publisher = {arXiv},
		year = {2021},
		doi = {10.48550/ARXIV.2105.08135},
		url = {https://arxiv.org/abs/2105.08135},
	}
	
% 	\bib{DLMSV}{article}{
%         AUTHOR = {De Lellis, Camillo},
%         author = {Marchese, Andrea},
%         author = {Spadaro, Emanuele},
%         author = {Valtorta, Daniele},
%         TITLE = {Rectifiability and upper {M}inkowski bounds for singularities
%               of harmonic {$Q$}-valued maps},
%         JOURNAL = {Comment. Math. Helv.},
%         %FJOURNAL = {Commentarii Mathematici Helvetici. A Journal of the Swiss
%         %      Mathematical Society},
%         VOLUME = {93},
%         YEAR = {2018},
%         NUMBER = {4},
%         PAGES = {737--779},
%         ISSN = {0010-2571},
%         % MRCLASS = {49Q20 (53A10 58A25)},
%         % MRNUMBER = {3880226},
%         % MRREVIEWER = {S\l awomir Kolasi\'{n}ski},
%         DOI = {10.4171/CMH/449},
%         URL = {https://doi.org/10.4171/CMH/449},
%     }
        
        \bib{DLSk1}{article}{
            AUTHOR = {De Lellis, Camillo},
            author = {Skorobogatova, Anna},
            TITLE = {On the singularity degree of area-minimizing integral currents at flat singular points},
        }
        
        \bib{DLSk2}{article}{
            AUTHOR = {De Lellis, Camillo},
            author = {Skorobogatova, Anna},
            TITLE = {Rectifiability of flat singularities of area minimizing integral currents: points with singularity degree strictly larger than $1$},
        }
        
    \bib{DLS_MAMS}{article}{
            AUTHOR = {De Lellis, Camillo},
            author={Spadaro, Emanuele Nunzio},
            TITLE = {{$Q$}-valued functions revisited},
            JOURNAL = {Mem. Amer. Math. Soc.},
            %FJOURNAL = {Memoirs of the American Mathematical Society},
            VOLUME = {211},
            YEAR = {2011},
            NUMBER = {991},
            PAGES = {vi+79},
            ISSN = {0065-9266},
            ISBN = {978-0-8218-4914-9},
            %MRCLASS = {49Q20 (35J50)},
            %MRNUMBER = {2663735},
            %MRREVIEWER = {Michele Miranda},
            DOI = {10.1090/S0065-9266-10-00607-1},
            URL = {https://doi.org/10.1090/S0065-9266-10-00607-1},
        }
        
        \bib{DLS_multiple_valued}{article}{
            AUTHOR = {De Lellis, Camillo},
            author={Spadaro, Emanuele},
            TITLE = {Multiple valued functions and integral currents},
            JOURNAL = {Ann. Sc. Norm. Super. Pisa Cl. Sci. (5)},
            %FJOURNAL = {Annali della Scuola Normale Superiore di Pisa. Classe di
                %Scienze. Serie V},
            VOLUME = {14},
            YEAR = {2015},
            NUMBER = {4},
            PAGES = {1239--1269},
            ISSN = {0391-173X},
            %MRCLASS = {49Q15 (49Q20)},
            %MRNUMBER = {3467655},
            %MRREVIEWER = {Luca Granieri},
        }
    \bib{DLS14Lp}{article}{
            AUTHOR = {De Lellis, Camillo},
            author = {Spadaro, Emanuele},
            TITLE = {Regularity of area minimizing currents {I}: gradient {$L^p$}
                estimates},
            JOURNAL = {Geom. Funct. Anal.},
            %FJOURNAL = {Geometric and Functional Analysis},
            VOLUME = {24},
            YEAR = {2014},
            NUMBER = {6},
            PAGES = {1831--1884},
            ISSN = {1016-443X},
            %MRCLASS = {49Q15 (49N60 49Q05)},
            %MRNUMBER = {3283929},
            %MRREVIEWER = {S\l awomir Kolasi\'{n}ski},
            DOI = {10.1007/s00039-014-0306-3},
            URL = {https://0-doi-org.pugwash.lib.warwick.ac.uk/10.1007/s00039-014-0306-3},
        }
        
        \bib{DLS16centermfld}{article}{
            AUTHOR = {De Lellis, Camillo},
            author={Spadaro, Emanuele},
            TITLE = {Regularity of area minimizing currents {II}: center manifold},
            JOURNAL = {Ann. of Math. (2)},
            %FJOURNAL = {Annals of Mathematics. Second Series},
            VOLUME = {183},
            YEAR = {2016},
            NUMBER = {2},
            PAGES = {499--575},
            ISSN = {0003-486X},
            %MRCLASS = {49Q15 (49Q05 53C42 58A20)},
            %MRNUMBER = {3450482},
            %MRREVIEWER = {S\l awomir Kolasi\'{n}ski},
            DOI = {10.4007/annals.2016.183.2.2},
            URL = {https://0-doi-org.pugwash.lib.warwick.ac.uk/10.4007/annals.2016.183.2.2},
        }
        
        
        \bib{DLS16blowup}{article}{
            AUTHOR = {De Lellis, Camillo},
            author = {Spadaro, Emanuele},
            TITLE = {Regularity of area minimizing currents {III}: blow-up},
            JOURNAL = {Ann. of Math. (2)},
            %FJOURNAL = {Annals of Mathematics. Second Series},
            VOLUME = {183},
            YEAR = {2016},
            NUMBER = {2},
            PAGES = {577--617},
            ISSN = {0003-486X},
            %MRCLASS = {49Q15 (53C42 58A20)},
            %MRNUMBER = {3450483},
            %MRREVIEWER = {S\l awomir Kolasi\'{n}ski},
            DOI = {10.4007/annals.2016.183.2.3},
            URL = {https://0-doi-org.pugwash.lib.warwick.ac.uk/10.4007/annals.2016.183.2.3},
        }
        
        \bib{DLSS1}{article}{
            AUTHOR = {De Lellis, Camillo},
            author={Spadaro, Emanuele},
            author={Spolaor, Luca},
            TITLE = {Regularity theory for {$2$}-dimensional almost minimal
                currents {I}: {L}ipschitz approximation},
            JOURNAL = {Trans. Amer. Math. Soc.},
            %FJOURNAL = {Transactions of the American Mathematical Society},
            VOLUME = {370},
            YEAR = {2018},
            NUMBER = {3},
            PAGES = {1783--1801},
            ISSN = {0002-9947},
            %MRCLASS = {49N60 (49Q05 49Q15)},
            %MRNUMBER = {3739191},
            %MRREVIEWER = {Martin Fuchs},
            DOI = {10.1090/tran/6995},
            URL = {https://doi.org/10.1090/tran/6995},
        }
        
        \bib{DLSS2}{article}{
            AUTHOR = {De Lellis, Camillo},
            author={Spadaro, Emanuele},
            author={Spolaor, Luca},
            TITLE = {Regularity theory for 2-dimensional almost minimal currents
                {II}: {B}ranched center manifold},
            JOURNAL = {Ann. PDE},
            %FJOURNAL = {Annals of PDE. Journal Dedicated to the Analysis of Problems
                %from Physical Sciences},
            VOLUME = {3},
            YEAR = {2017},
            NUMBER = {2},
            PAGES = {Paper No. 18, 85},
            ISSN = {2524-5317},
            %MRCLASS = {49Q15 (49N15 58A25)},
            %MRNUMBER = {3712561},
            %MRREVIEWER = {Laurent Moonens},
            DOI = {10.1007/s40818-017-0035-7},
            URL = {https://doi.org/10.1007/s40818-017-0035-7},
        }
        \bib{DLSS3}{article}{
            AUTHOR = {De Lellis, Camillo},
            author={Spadaro, Emanuele},
            author={Spolaor, Luca},
            TITLE = {Regularity theory for 2-dimensional almost minimal currents
                {III}: {B}lowup},
            JOURNAL = {J. Differential Geom.},
            %FJOURNAL = {Journal of Differential Geometry},
            VOLUME = {116},
            YEAR = {2020},
            NUMBER = {1},
            PAGES = {125--185},
            ISSN = {0022-040X},
            %MRCLASS = {49N60 (49Q15 49Q20 58A25)},
            %MRNUMBER = {4146358},
            DOI = {10.4310/jdg/1599271254},
            URL = {https://doi.org/10.4310/jdg/1599271254},
        }
        
        \bib{Hardt_Simon_boundary}{article}{
            AUTHOR = {Hardt, Robert},
            author={Simon, Leon},
            TITLE = {Boundary regularity and embedded solutions for the oriented
                {P}lateau problem},
            JOURNAL = {Ann. of Math. (2)},
            %FJOURNAL = {Annals of Mathematics. Second Series},
            VOLUME = {110},
            YEAR = {1979},
            NUMBER = {3},
            PAGES = {439--486},
            ISSN = {0003-486X},
            %MRCLASS = {49F10 (49F20 53A10)},
            %MRNUMBER = {554379},
            %MRREVIEWER = {Jo\~{a}o Lucas Marques Barbosa},
            DOI = {10.2307/1971233},
            URL = {https://doi.org/10.2307/1971233},
        }
        
        \bib{Federer}{book}{
            AUTHOR = {Federer, Herbert},
            TITLE = {Geometric measure theory},
            SERIES = {Die Grundlehren der mathematischen Wissenschaften, Band 153},
            PUBLISHER = {Springer-Verlag New York Inc., New York},
            YEAR = {1969},
            PAGES = {xiv+676},
            %MRCLASS = {28.80 (26.00)},
            %MRNUMBER = {0257325},
            %MRREVIEWER = {J. E. Brothers},
        }
        
        \bib{Federer1970}{article}{
            AUTHOR = {Federer, Herbert},
            TITLE = {The singular sets of area minimizing rectifiable currents with
                codimension one and of area minimizing flat chains modulo two
                with arbitrary codimension},
            JOURNAL = {Bull. Amer. Math. Soc.},
            %FJOURNAL = {Bulletin of the American Mathematical Society},
            VOLUME = {76},
            YEAR = {1970},
            PAGES = {767--771},
            ISSN = {0002-9904},
            %MRCLASS = {28.80 (26.00)},
            %MRNUMBER = {260981},
            %MRREVIEWER = {J. E. Brothers},
            DOI = {10.1090/S0002-9904-1970-12542-3},
            URL = {https://doi.org/10.1090/S0002-9904-1970-12542-3},
        }

        \bib{Liu}{article}{
  AUTHOR = {Liu, Zhenhua},
  TITLE = {On a conjecture of Almgren: area-minimizing surfaces with fractal singularities},
  JOURNAL = {arXiv preprint},
  YEAR = {2021},
  DOI = {10.48550/ARXIV.2110.13137},
  URL = {https://arxiv.org/abs/2110.13137}
}
        
        \bib{NV_Annals}{article}{
             AUTHOR = {Naber, Aaron},
             author={Valtorta, Daniele},
             TITLE = {Rectifiable-{R}eifenberg and the regularity of stationary and
                 minimizing harmonic maps},
             JOURNAL = {Ann. of Math. (2)},
             %FJOURNAL = {Annals of Mathematics. Second Series},
             VOLUME = {185},
             YEAR = {2017},
             NUMBER = {1},
             PAGES = {131--227},
             ISSN = {0003-486X},
             %MRCLASS = {58E20 (53C43)},
             %MRNUMBER = {3583353},
             %MRREVIEWER = {Andreas Gastel},
             DOI = {10.4007/annals.2017.185.1.3},
             URL = {https://doi.org/10.4007/annals.2017.185.1.3},
         }

                 \bib{NV_varifolds}{article}{
             AUTHOR = {Naber, Aaron},
             author = {Valtorta, Daniele},
             TITLE = {The singular structure and regularity of stationary varifolds},
             JOURNAL = {J. Eur. Math. Soc. (JEMS)},
             %FJOURNAL = {Journal of the European Mathematical Society (JEMS)},
             VOLUME = {22},
             YEAR = {2020},
             NUMBER = {10},
             PAGES = {3305--3382},
             ISSN = {1435-9855},
             %MRCLASS = {58E12 (35J60 35J93 49Q20)},
             %MRNUMBER = {4153109},
             %MRREVIEWER = {Pei Biao Zhao},
             DOI = {10.4171/jems/987},
             URL = {https://doi.org/10.4171/jems/987},
        }
        
            \bib{Simon_rect}{article}{
            AUTHOR = {Simon, Leon},
            TITLE = {Rectifiability of the singular sets of multiplicity {$1$}
                minimal surfaces and energy minimizing maps},
            BOOKTITLE = {Surveys in differential geometry, {V}ol. {II} ({C}ambridge,
                {MA}, 1993)},
            PAGES = {246--305},
            PUBLISHER = {Int. Press, Cambridge, MA},
            YEAR = {1995},
            %MRCLASS = {49Q05 (58E12)},
            %MRNUMBER = {1375258},
            %MRREVIEWER = {Martin Fuchs},
        }
    
    	\bib{Simon_cylindrical}{article}{
    		author = {Leon Simon},
    		title = {{Cylindrical tangent cones and the singular set of minimal submanifolds}},
    		volume = {38},
    		journal = {Journal of Differential Geometry},
    		number = {3},
    		publisher = {Lehigh University},
    		pages = {585 -- 652},
    		year = {1993},
    		doi = {10.4310/jdg/1214454484},
    		URL = {https://doi.org/10.4310/jdg/1214454484}
    	}
    	
        
        % \bib{Simon_GMT}{book}{
        %     AUTHOR = {Simon, Leon},
        %     TITLE = {Lectures on geometric measure theory},
        %     SERIES = {Proceedings of the Centre for Mathematical Analysis,
        %       Australian National University},
        %     VOLUME = {3},
        %     PUBLISHER = {Australian National University, Centre for Mathematical
        %       Analysis, Canberra},
        %     YEAR = {1983},
        %     PAGES = {vii+272},
        %     ISBN = {0-86784-429-9},
        %     %MRCLASS = {49-01 (28A75 49F20)},
        %     %MRNUMBER = {756417},
        %     %MRREVIEWER = {J. S. Joel},
        % }
        
        \bib{Sk21}{article}{
            title={An upper Minkowski bound for the interior singular set of area minimizing currents}, 
            author={Skorobogatova, Anna},
            year={2021},
            eprint={2108.00418},
            %archivePrefix={arXiv},
            %primaryClass={math.DG}
        }
        
        % \bib{Spolaor_15}{article}{
        %     AUTHOR = {Spolaor, Luca},
        %     TITLE = {Almgren's type regularity for semicalibrated currents},
        %     JOURNAL = {Adv. Math.},
        %     %FJOURNAL = {Advances in Mathematics},
        %     VOLUME = {350},
        %     YEAR = {2019},
        %     PAGES = {747--815},
        %     ISSN = {0001-8708},
        %     %MRCLASS = {49Q15 (49N60)},
        %     %MRNUMBER = {3948685},
        %     %MRREVIEWER = {Alp\'{a}r R. M\'{e}sz\'{a}ros},
        %     DOI = {10.1016/j.aim.2019.04.057},
        %     URL = {https://doi.org/10.1016/j.aim.2019.04.057},
        % }
        
        % \bib{WhiteStrat}{article}{
        %     AUTHOR = {White, Brian},
        %     TITLE = {Stratification of minimal surfaces, mean curvature flows, and
        %         harmonic maps},
        %     JOURNAL = {J. Reine Angew. Math.},
        %     %FJOURNAL = {Journal f\"{u}r die Reine und Angewandte Mathematik. [Crelle's
        %     %    Journal]},
        %     VOLUME = {488},
        %     YEAR = {1997},
        %     PAGES = {1--35},
        %     ISSN = {0075-4102},
        %     %MRCLASS = {49Q05 (49Q20 53C42 58E20)},
        %     %MRNUMBER = {1465365},
        %     %MRREVIEWER = {Harold Parks},
        %     DOI = {10.1515/crll.1997.488.1},
        %     URL = {https://doi.org/10.1515/crll.1997.488.1},
        % }

        \bib{White}{article}{
        AUTHOR = {White, Brian},
        TITLE = {Tangent cones to two-dimensional area-minimizing integral
              currents are unique},
        JOURNAL = {Duke Math. J.},
        %FJOURNAL = {Duke Mathematical Journal},
        VOLUME = {50},
        YEAR = {1983},
        NUMBER = {1},
        PAGES = {143--160},
        ISSN = {0012-7094},
        %MRCLASS = {49F22 (49F10)},
        %MRNUMBER = {700134},
        DOI = {10.1215/S0012-7094-83-05005-6},
        URL = {https://doi.org/10.1215/S0012-7094-83-05005-6},
        }

    	\bib{W14_annals}{article}{
    		title={A general regularity theory for stable codimension 1 integral varifolds},
    		author={Wickramasekera, Neshan},
    		journal={Annals of mathematics},
    		pages={843--1007},
    		year={2014}
    	}
    	
    	    \bib{Morgan}{article}{
    AUTHOR = {Morgan, Frank},
     TITLE = {On the singular structure of two-dimensional area minimizing
              surfaces in {${\bf R}^{n}$}},
   JOURNAL = {Math. Ann.},
  %FJOURNAL = {Mathematische Annalen},
    VOLUME = {261},
      YEAR = {1982},
    NUMBER = {1},
     PAGES = {101--110},
      ISSN = {0025-5831},
   %MRCLASS = {49F22},
  %MRNUMBER = {675210},
%MRREVIEWER = {Jean E. Taylor},
       DOI = {10.1007/BF01456413},
       URL = {https://doi.org/10.1007/BF01456413},
}

\bib{KW}{article}{
  author = {Krummel, Brian},
  author = {Wickramasekera, Neshan},
  title = {Fine properties of branch point singularities: Dirichlet energy minimizing multi-valued functions},
  publisher = {arXiv},
  year = {2017},
    doi = {10.48550/ARXIV.1711.06222},
    url = {https://arxiv.org/abs/1711.06222},
}

    	
    \end{biblist}
\end{bibdiv}

==> comments-remarks.tex <==
1) Combinatorial lemmas: should we try to ``unify'' them?

2) Tilt-excess decay, how much of the proof depends on the area-minimizing assumption?

{\color{orange}[P: Just as a comment to think about: how much of this height bound do we actually need area-minimizing for? A lot of the argument seems to go through without assuming this. One place it does seem to be used is in bounding the oriented tilt by the non-oriented tilt, however if one allows themselves to just work with the non-oriented tilt everywhere, can one do this?]}
\note{A: yep to bound $\Ebf$ by $\Ebf^{no}$ we indeed heavily rely on area-minimizing, but I agree that if one consistently works with non-oriented tilt throughout, it seems like we get the same conclusions (obviously with the tilt-excess bound on $\Ebf^{no}$). Maybe it's worth adding this as a remark}
{\color{blue}[C: Paul, why do you think we can remove the first term from (5.10)? To me it seems it is needed. As for the question about where we actually need area-minimizing: in the estimate of Lemma 5.1 we are using Almgren's estimate to gain the superlinear power on the term which is ``undesirable'' and which later gets eliminated. That is really something which we only know how to do in the area-minimizing case and a few conversation back with Ulrich Menne he convinced me it's false on a stationary varifold. His point was that with a rescaled catenoid you can show that you can only gain a log... although you might object that the catenoid is not really a valid counterexample to the estimate because it does not project to a double cover of the plane. At any rate it might be that we don't really need to gain the superlinear power but just a linear estimate with a small constant in front: this is what I thought at first and I wanted to use some old lemma of De Giorgi which would have needed an infinite iteration and a careful choice of the radii. I then noticed that I could iterate a finite number of times because we gain a power.]}

{\color{orange} [P: Regarding the stationary case, I agree -- I'm not quite sure how I missed the application in Lemma 5.1!]}
\note{A: Ah yep I also completely overlooked the use of the higher integrability of the graphical approximation for $T$ in Almgren's excess estimate that is used in the proof of Lemma 5.1...}

3) Do the Morgan angles of pairs of m-planes with (m-2)-dimensional intersection coincide in the Dir-minimizing situation?

4) {\color{orange}[P: This should be moved to our comments/remark folder, but just so people see it: we really don't seem to be using the full structure of the assumptions in Proposition 7.5 to get this result, namely the assumption that all the planes have the same $(m-2)$-subspace $V$ doesn't seem to be relevant. At the very least, it seems that you could prove the same comparability between the Morgan angles for a Dir-minimizer which is a union of planes, provided each pair of planes intersects along a set which is $(m-2)$-dimensional. Do people agree? Even then, the only place where we use the $(m-2)$-dimensional intersection seems to be in Lemma 7.6, otherwise we contradict the regularity theory. Even in a more general situation, one should still be able to prove that the maximum Morgan angle is comparable to the second largest Morgan angle, by the same proof, no? It seems perhaps that you cannot say anymore than that, but perhaps it would be good to remark this?]} {\color{blue} Indeed, agree on all the line and probably worth a remark. After Anna sees the discussion and expresses an opinion, I'll move the thread to the comments/remark folder.}
\note{I agree also, and I think it's worthwhile remarking this}
